The VLA/ALMA Nascent Disk and Multiplicity (VANDAM) Survey of Orion Protostars IV. Unveiling the Embedded Intermediate-Mass Protostar and Disk within OMC2-FIR3/HOPS-370

We present ALMA (0.87~mm and 1.3~mm) and VLA (9~mm) observations toward the candidate intermediate-mass protostar OMC2-FIR3 (HOPS-370; L$_{bol}$~314~L$_{\odot}$) at $\sim$0.1" (40~au) resolution for the continuum emission and ~0.25" (100 au) resolution of nine molecular lines. The dust continuum observed with ALMA at 0.87~mm and 1.3~mm resolve a near edge-on disk toward HOPS-370 with an apparent radius of ~100 au. The VLA observations detect both the disk in dust continuum and free-free emission extended along the jet direction. The ALMA observations of molecular lines (H$_2$CO, SO, CH$_3$OH, $^{13}$CO, C$^{18}$O, NS, and H$^{13}$CN) reveal rotation of the apparent disk surrounding HOPS-370 orthogonal to the jet/outflow direction. We fit radiative transfer models to both the dust continuum structure of the disk and molecular line kinematics of the inner envelope and disk for the H$_2$CO, CH$_3$OH, NS, and SO lines. The central protostar mass is determined to be $\sim$2.5 M_sun with a disk radius of $\sim$94~au, when fit using combinations of the H$_2$CO, CH$_3$OH, NS, and SO lines, consistent with an intermediate-mass protostar. Modeling of the dust continuum and spectral energy distribution (SED) yields a disk mass of 0.035~M$_{\odot}$ (inferred dust+gas) and a dust disk radius of 62~au, thus the dust disk may have a smaller radius than the gas disk, similar to Class II disks. In order to explain the observed luminosity with the measured protostar mass, HOPS-370 must be accreting at a rate between 1.7 and 3.2$\times$10$^{-5}$~M$_{\odot}$~yr$^{-1}$.

==> tab8.tex <==
\begin{deluxetable}{lllllllllllllll}
\rotate
\tabletypesize{\tiny}
\tablewidth{0pt}
\tablecaption{HOPS-370 Molecular Line Models - Exponentially Tapered Disks with Envelope}
\tablehead{\colhead{Transition(s)} & \colhead{Mass} & \colhead{Disk Radius} & \colhead{Disk Mass} & \colhead{Envelope Radius} & \colhead{Envelope Mass}  & \colhead{V$_{lsr}$}     & \colhead{Pos. Angle} & \colhead{$\Delta$x} & \colhead{$\Delta$y}  & \colhead{$\gamma$} & \colhead{T(1 au)} & \colhead{q} & \colhead{$log_{10}$(Mol./H$_2$)\tablenotemark{b}}\\
                                   & \colhead{(M$_{\sun}$)} & \colhead{(AU)} & \colhead{(M$_{\sun}$)} & \colhead{(AU)} & \colhead{(M$_{\sun}$)} & \colhead{(km~s$^{-1}$)} & \colhead{\degr}      & \colhead{(\arcsec)} & \colhead{(\arcsec)} &                              &       (K)     &                 &
}
\startdata
%                CH$_3$OH ($J=4_{2,2}\rightarrow3_{1,2}$) & 2.39$\pm$0.03 & 140.73$\pm$1.56 & 10.99$\pm$0.03 & 357.72$\pm$0.65 & 0.01$\pm$0.002 & 0.01$\pm$0.002 & 0.40$\pm$0.03 & 0.35\\
%                      SO ($J_N = 6_5\rightarrow5_4$) & 2.65$\pm$0.04 & 83.75$\pm$1.01 & 11.51$\pm$0.02 & 343.73$\pm$0.64 & 0.02$\pm$0.002 & 0.03$\pm$0.002 & 1.09$\pm$0.01 & 0.35\\
%SO\tablenotemark{a} and CH$_3$OH \\
%NS\\
%NS\tablenotemark{a} and CH$_3$OH\\
%NS and SO\tablenotemark{a}\\
%      H$_2$CO (3 lines) & 2.43$\pm$0.02 & 137.91$\pm$0.93 & 11.02$\pm$0.01 & 353.73$\pm$0.25 & 0.01$\pm$0.001 & 0.02$\pm$0.001 & 0.52$\pm$0.01 & 0.35\\
%             H$_2$CO (3 lines, q fit) & 2.50$\pm$0.02 & 136.10$\pm$0.86 & 11.03$\pm$0.01 & 353.42$\pm$0.29 & 0.01$\pm$0.001 & 0.02$\pm$0.001 & 0.54$\pm$0.01 & 0.39$\pm$0.01\\
%               H$_2$CO (2 lines) & 2.26$\pm$0.03 & 123.42$\pm$1.26 & 11.03$\pm$0.02 & 353.80$\pm$0.33 & 0.01$\pm$0.002 & 0.02$\pm$0.002 & 0.74$\pm$0.01 & 0.35\\
%               H$_2$CO ($J=3_{0,3}\rightarrow2_{0,2}$) & 2.86$\pm$0.05 & 92.26$\pm$0.88 & 11.10$\pm$0.02 & 353.32$\pm$0.43 & 0.01$\pm$0.002 & 0.02$\pm$0.002 & 0.91$\pm$0.02 & 0.35\\
%              SO, H$_2$CO (3 lines) & 2.31$\pm$0.02 & 112.13$\pm$0.59 & 11.07$\pm$0.01 & 353.32$\pm$0.27 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 0.63$\pm$0.01 & 0.35\\
%   SO\tablenotemark{a}, H$_2$CO (3 lines) & 2.38$\pm$0.02 & 130.25$\pm$0.80 & 11.05$\pm$0.01 & 352.80$\pm$0.43 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 0.54$\pm$0.01 & 0.35 & -8.69$\pm$0.00\\
%  NS\tablenotemark{a}, H$_2$CO (3 lines)\\
%   CH$_3$OH\tablenotemark{a}, H$_2$CO (3 lines)\\
  H$_2$CO ($J=3_{0,3}\rightarrow2_{0,2}$) & 2.81$\pm$0.03 & 32.97$\pm$3.3 & 0.77$\pm$0.070 & 8345.89$\pm$8536.0 & 0.548$\pm$0.660 & 11.19$\pm$0.02 & 353.35$\pm$0.34 & -0.000$\pm$0.002 & 0.015$\pm$0.001 & 1.32$\pm$0.02 & 997.43$\pm$3.76 & 0.35 & \nodata  \\ 
                        H$_2$CO (2 lines) & 2.46$\pm$0.03 & 36.07$\pm$4.1 & 0.85$\pm$0.075 & 1081.80$\pm$182.1 & 0.049$\pm$0.010 & 11.21$\pm$0.02 & 352.00$\pm$0.44 & 0.011$\pm$0.002 & 0.004$\pm$0.002 & 1.37$\pm$0.03 & 998.69$\pm$1.66 & 0.35 & \nodata  \\ 
                        H$_2$CO (3 lines) & 2.66$\pm$0.02 & 62.99$\pm$3.1 & 0.69$\pm$0.034 & 1076.49$\pm$21.0 & 0.071$\pm$0.004 & 11.20$\pm$0.01 & 352.39$\pm$0.28 & 0.006$\pm$0.001 & 0.009$\pm$0.001 & 1.16$\pm$0.02 & 999.52$\pm$0.66 & 0.35 & \nodata  \\ 
 CH$_3$OH ($J=4_{2,2}\rightarrow3_{1,2}$) & 2.46$\pm$0.03 & 81.51$\pm$5.6 & 0.51$\pm$0.035 & 1009.67$\pm$20.1 & 0.037$\pm$0.004 & 11.07$\pm$0.02 & 357.55$\pm$0.54 & 0.012$\pm$0.002 & -0.001$\pm$0.002 & 1.08$\pm$0.04 & 998.72$\pm$1.91 & 0.35 & \nodata  \\ 
 CH$_3$OH\tablenotemark{a}, H$_2$CO (3 lines) & 2.60$\pm$0.02 & 74.65$\pm$2.5 & 0.57$\pm$0.019 & 1013.96$\pm$29.7 & 0.054$\pm$0.002 & 11.14$\pm$0.01 & 353.58$\pm$0.22 & 0.007$\pm$0.001 & 0.008$\pm$0.001 & 1.09$\pm$0.02 & 999.09$\pm$0.85 & 0.35 & -7.99$\pm$0.005  \\ 
           SO ($J_N = 6_5\rightarrow5_4$) & 2.63$\pm$0.04 & 90.16$\pm$4.1 & 0.23$\pm$0.011 & 1013.35$\pm$15.2 & 0.013$\pm$0.001 & 11.53$\pm$0.02 & 344.85$\pm$0.61 & 0.024$\pm$0.002 & 0.036$\pm$0.002 & 1.00$\pm$0.05 & 999.36$\pm$0.73 & 0.35 & \nodata  \\ 
         SO\tablenotemark{a} and CH$_3$OH & 2.35$\pm$0.04 & 113.69$\pm$2.9 & 0.30$\pm$0.012 & 1067.64$\pm$35.0 & 0.023$\pm$0.003 & 11.12$\pm$0.03 & 352.97$\pm$0.65 & 0.013$\pm$0.001 & 0.026$\pm$0.002 & 0.65$\pm$0.04 & 993.91$\pm$3.08 & 0.35 & -8.70$\pm$0.007  \\ 
   SO\tablenotemark{a}, H$_2$CO (3 lines) & 2.63$\pm$0.02 & 85.17$\pm$2.4 & 0.50$\pm$0.015 & 5466.58$\pm$202.3 & 0.320$\pm$0.026 & 11.19$\pm$0.01 & 351.38$\pm$0.23 & 0.009$\pm$0.001 & 0.015$\pm$0.001 & 1.02$\pm$0.02 & 999.23$\pm$0.88 & 0.35 & -8.76$\pm$0.005  \\ 
                                       NS & 3.83$\pm$0.15 & 55.96$\pm$26.9 & 0.03$\pm$0.018 & 5889.31$\pm$3114.6 & 0.046$\pm$0.067 & 11.01$\pm$0.07 & 350.24$\pm$1.52 & -0.010$\pm$0.004 & 0.013$\pm$0.003 & 0.55$\pm$0.35 & 424.31$\pm$38.63 & 0.35 & \nodata  \\ 
                  NS, SO\tablenotemark{a} & 1.85$\pm$0.03 & 14.17$\pm$2.2 & 0.06$\pm$0.004 & 4671.31$\pm$117.8 & 0.006$\pm$0.002 & 11.10$\pm$0.03 & 353.53$\pm$0.55 & 0.018$\pm$0.002 & 0.060$\pm$0.002 & 1.57$\pm$0.02 & 998.54$\pm$1.37 & 0.35 & -7.50$\pm$0.002  \\ 
            NS\tablenotemark{a}, CH$_3$OH & 2.52$\pm$0.04 & 88.72$\pm$6.8 & 0.46$\pm$0.035 & 1074.55$\pm$180.6 & 0.029$\pm$0.007 & 11.07$\pm$0.03 & 356.83$\pm$0.66 & 0.009$\pm$0.003 & 0.004$\pm$0.002 & 1.04$\pm$0.05 & 991.41$\pm$4.22 & 0.35 & -9.77$\pm$0.018  \\ 
   NS\tablenotemark{a}, H$_2$CO (3 lines) & 2.67$\pm$0.02 & 78.74$\pm$2.7 & 0.55$\pm$0.021 & 5475.02$\pm$481.8 & 0.532$\pm$0.066 & 11.17$\pm$0.01 & 352.43$\pm$0.31 & 0.006$\pm$0.001 & 0.010$\pm$0.001 & 1.07$\pm$0.02 & 998.17$\pm$1.80 & 0.35 & -9.82$\pm$0.018  \\ 
                 H$_2$CO (3 lines, q fit) & 2.57$\pm$0.02 & 52.98$\pm$0.9 & 0.99$\pm$0.011 & 1054.51$\pm$15.0 & 0.18$\pm$0.005 & 11.33$\pm$0.01 & 352.71$\pm$0.26 & 0.004$\pm$0.001 & 0.003$\pm$0.001 & 1.27$\pm$0.01 & 998.85$\pm$1.46 & 0.0003$\pm$0.0005 & \nodata  \\ 
%\hline
%Non-Continuum-subtracted Models\\
%\hline
%                        CH$_3$OH ($J=4_{2,2}\rightarrow3_{1,2}$) & 2.24$\pm$0.03 & 135.99$\pm$1.28 & 10.95$\pm$0.03 & 360.94$\pm$0.57 & 0.01$\pm$0.002 & 0.01$\pm$0.002 & 0.65$\pm$0.02 & 0.35 \\
%                           SO ($J_N = 6_5\rightarrow5_4$) & 1.72$\pm$0.02 & 60.74$\pm$0.80 & 11.03$\pm$0.02 & 352.56$\pm$0.57 & 0.02$\pm$0.002 & 0.07$\pm$0.002 & 1.28$\pm$0.01 & 0.35 \\
%               H$_2$CO (3 lines) & 2.51$\pm$0.02 & 133.30$\pm$0.40 & 10.99$\pm$0.01 & 354.75$\pm$0.33 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 0.61$\pm$0.01 & 0.35 \\
%                     H$_2$CO (3 lines, q fit) & 2.64$\pm$0.02 & 136.09$\pm$1.04 & 10.99$\pm$0.01 & 354.50$\pm$0.26 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 0.55$\pm$0.02 & 0.50$\pm$0.00\\
%                       H$_2$CO (2 lines) & 2.49$\pm$0.03 & 114.17$\pm$1.54 & 11.03$\pm$0.01 & 354.10$\pm$0.45 & 0.01$\pm$0.002 & 0.02$\pm$0.002 & 0.81$\pm$0.02 & 0.35 \\
%                       H$_2$CO ($J=3_{0,3}\rightarrow2_{0,2}$) & 3.13$\pm$0.03 & 94.72$\pm$1.63 & 11.05$\pm$0.01 & 353.73$\pm$0.25 & 0.01$\pm$0.002 & 0.03$\pm$0.001 & 0.79$\pm$0.02 & 0.35 \\
%                      SO, H$_2$CO (3 lines) & 2.29$\pm$0.02 & 104.40$\pm$0.87 & 10.95$\pm$0.01 & 355.67$\pm$0.31 & 0.01$\pm$0.001 & 0.04$\pm$0.001 & 0.70$\pm$0.02 & 0.35 \\
%           SO, H$_2$CO (3 lines; SO abund. fit) & 2.16$\pm$0.02 & 123.11$\pm$0.78 & 10.92$\pm$0.01 & 356.42$\pm$0.30 & 0.01$\pm$0.001 & 0.05$\pm$0.001 & 0.84$\pm$0.01  & 0.35 & -8.71$\pm$0.00\\
\enddata
%\hline
%Truncated Disks\\
%\hline
%                      ch3oh-model0-trunc & 2.13$\pm$0.15 & 225.14$\pm$15.48 & 10.91$\pm$0.08 & 362.86$\pm$1.96 & 0.01$\pm$0.003 & 0.01$\pm$0.007 & 1.22$\pm$0.48\\
%              ch3oh-model0-trunc-contsub & 2.49$\pm$0.03 & 176.35$\pm$0.98 & 11.09$\pm$0.02 & 358.24$\pm$0.44 & 0.00$\pm$0.002 & -0.01$\pm$0.002 & 0.03$\pm$0.03\\
%                         so-model3-trunc & 1.79$\pm$0.02 & 173.66$\pm$1.20 & 10.95$\pm$0.02 & 353.91$\pm$0.44 & 0.01$\pm$0.002 & 0.06$\pm$0.002 & 0.69$\pm$0.05\\
%                 so-model3-trunc-contsub & 2.78$\pm$0.03 & 161.48$\pm$0.20 & 11.56$\pm$0.02 & 348.92$\pm$0.49 & 0.01$\pm$0.002 & 0.03$\pm$0.002 & 0.00$\pm$0.00\\
%             h2co-all-model0-trunc-fix-q & 2.59$\pm$0.02 & 268.58$\pm$8.55 & 11.07$\pm$0.01 & 352.47$\pm$0.37 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 1.22$\pm$0.06\\
%     h2co-all-model0-trunc-fix-q-contsub & 2.66$\pm$0.02 & 254.52$\pm$0.42 & 11.05$\pm$0.01 & 352.56$\pm$0.35 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 1.21$\pm$0.02\\
%                     h2co-h-model0-trunc & 2.44$\pm$0.03 & 254.91$\pm$0.31 & 11.08$\pm$0.02 & 352.05$\pm$0.41 & 0.01$\pm$0.002 & 0.03$\pm$0.002 & 1.39$\pm$0.03\\
%             h2co-h-model0-trunc-contsub & 2.20$\pm$0.02 & 255.24$\pm$0.13 & 11.07$\pm$0.02 & 352.03$\pm$0.41 & 0.01$\pm$0.002 & 0.02$\pm$0.002 & 1.40$\pm$0.01\\
%                     h2co-l-model0-trunc & 3.14$\pm$0.03 & 250.28$\pm$0.48 & 11.11$\pm$0.01 & 351.75$\pm$0.31 & 0.00$\pm$0.002 & 0.03$\pm$0.001 & 1.21$\pm$0.04\\
%             h2co-l-model0-trunc-contsub & 3.32$\pm$0.03 & 248.22$\pm$0.38 & 11.16$\pm$0.01 & 350.73$\pm$0.28 & 0.00$\pm$0.002 & 0.02$\pm$0.002 & 0.95$\pm$0.04\\
%                     so-h2co-model0-trunc & 2.46$\pm$0.03 & 224.02$\pm$0.73 & 11.03$\pm$0.02 & 353.38$\pm$0.39 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 1.02$\pm$0.02\\
%            so-h2co-model0-trunc-contsub & 2.64$\pm$0.02 & 203.64$\pm$0.04 & 11.05$\pm$0.01 & 351.61$\pm$0.24 & 0.01$\pm$0.001 & 0.02$\pm$0.001 & 0.51$\pm$0.02\\
%         so-h2co-model0-trunc-so-abundvar & 2.45$\pm$0.22 & 204.14$\pm$21.79 & 10.99$\pm$0.03 & 354.30$\pm$0.59 & 0.01$\pm$0.002 & 0.03$\pm$0.009 & 0.83$\pm$0.31 & -8.02$\pm$0.34\\
% so-h2co-model0-trunc-so-abundvar-contsub & 2.39$\pm$0.03 & 250.85$\pm$0.30 & 11.08$\pm$0.01 & 351.28$\pm$0.19 & 0.01$\pm$0.001 & 0.03$\pm$0.001 & 1.25$\pm$0.01 & -8.68$\pm$0.00\\
\tablecomments{The results from each model lists the molecular line(s) fit with the \textit{pdspy} models.
For H$_2$CO, `3 lines', refers to all three ($J=3_{n,n}\rightarrow2_{n,n}$) transitions, while `2 lines' refers to the higher
excitation ($J=3_{2,2}\rightarrow2_{2,1}$) and ($J=3_{2,1}\rightarrow2_{2,0}$) transitions (see Table 1). The parameter
$q$, the power-law index of the disk 
temperature profile is fixed for all models except when `q fit' is listed in the description.
The Mass column refers to the protostar mass, $\Delta x$ and $\Delta y$ refer to the offset of the
model center of mass with respect to the image phase center, $\gamma$ is the power-law index of the 
disk surface density profile, and SO Abund. refers to the SO abundance adopted or fit by the models.}
\tablenotetext{a}{Abundance of denoted molecule was allowed to vary as part of the fitting process to enable
better convergence.}
\tablenotetext{b}{Abundance provided is for the molecule in the first column that have a superscript a.}
\end{deluxetable}

